Sheaves, Cosheaves and Applications

This thesis develops the theory of sheaves and cosheaves with an eye towards applications in science and engineering. To provide a theory that is computable, we focus on a combinatorial version of sheaves and cosheaves called cellular sheaves and cosheaves, which are finite families of vector spaces and maps parametrized by a cell complex. We develop cellular (co)sheaves as a new tool for topological data analysis, network coding and sensor networks. A foundation for multi-dimensional level-set persistent homology is laid via constructible cosheaves, which are equivalent to representations of MacPherson's entrance path category. By proving a van Kampen theorem, we give a direct proof of this equivalence. A cosheaf version of the i'th derived pushforward of the constant sheaf along a definable map is constructed directly as a representation of this category. We go on to clarify the relationship of cellular sheaves to cosheaves by providing a formula that defines a derived equivalence, which in turn recovers Verdier duality. Compactly-supported sheaf cohomology is expressed as the coend with the image of the constant sheaf through this equivalence. The equivalence is further used to establish relations between sheaf cohomology and a herein newly introduced theory of cellular sheaf homology. Inspired to provide fast algorithms for persistence, we prove that the derived category of cellular sheaves over a 1D cell complex is equivalent to a category of graded sheaves. Finally, we introduce the interleaving distance as an extended pseudo-metric on the category of sheaves. We prove that global sections partition the space of sheaves into connected components. We conclude with an investigation into the geometry of the space of constructible sheaves over the real line, which we relate to the bottleneck distance in persistence.

==> THESIS_shortcuts.tex <==
%%%%%%%%%%%%%%%Justin's shortcuts, inspired by Vidit

% THEOREMS
\theoremstyle{definition}
\newtheorem{thm}{Theorem}[section]
\newtheorem{lem}[thm]{Lemma}
\newtheorem{defn}[thm]{Definition}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{ex}[thm]{Example}
\newtheorem{rem}[thm]{Remark}
\newtheorem{rmk}[thm]{Remark}
\newtheorem{exer}[thm]{Exercise}
\newtheorem{alg}[thm]{Algorithm}
\newtheorem{com}[thm]{Comment}
\newtheorem{conj}[thm]{Conjecture}
\newtheorem{quest}[thm]{Question}
\newtheorem{clm}[thm]{Claim}
\newtheorem{exr}[thm]{Exercise}

\renewcommand{\sfdefault}{iwona}
\DeclareMathAlphabet{\mathbfsf}{\encodingdefault}{\sfdefault}{bx}{n}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\dd}{\dagger}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%    CATEGORIES  %%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \newcommand{\Hom}{\mathsf{Hom}}
% \newcommand{\obj}{\mathsf{obj}}
% \newcommand{\mor}{\mathsf{mor}}
% \newcommand{\Obj}{\mathsf{Obj}}
% \newcommand{\Mor}{\mathsf{Mor}}
% \newcommand{\Nat}{\mathsf{Nat}}
% \newcommand{\Grp}{\mathsf{Grp}}
% \newcommand{\Grpd}{\mathsf{Grpd}}
% \newcommand{\SSet}{\mathsf{SSet}}
% \newcommand{\Set}{\mathsf{Set}}
% \newcommand{\Rel}{\mathsf{Rel}}
% \newcommand{\Vect}{\mathsf{Vect}}
% \newcommand{\vect}{\mathsf{vect}}
% \newcommand{\Hilb}{\mathsf{Hilb}}
% \newcommand{\Cat}{\mathsf{Cat}}
% \newcommand{\Top}{\mathsf{Top}}
% \newcommand{\hoTop}{\mathsf{hoTop}}
% \newcommand{\Fun}{\mathsf{Fun}}
% \newcommand{\Ab}{\mathsf{Ab}}
% \newcommand{\Cov}{\mathsf{Cov}}
% \newcommand{\Fincov}{\mathsf{FinCov}}
% \newcommand{\Cell}{\mathsf{Cell}}
% \newcommand{\Open}{\mathsf{Open}}
% \newcommand{\Closed}{\mathsf{Closed}}
% \newcommand{\Int}{\mathsf{Int}}
% \newcommand{\Exit}{\mathsf{Exit}}
% \newcommand{\Entr}{\mathsf{Entr}}
% \newcommand{\Rep}{\mathsf{Rep}}
% \newcommand{\Shv}{\mathsf{Shv}}
% \newcommand{\Coshv}{\mathsf{CoShv}}
% \newcommand{\Rout}{\mathsf{Rout}}
% \newcommand{\Cone}{\mathsf{Cone}}
% \newcommand{\CoCone}{\mathsf{CoCone}}
% \newcommand{\Alex}{\mathsf{Alex}}
% \newcommand{\Free}{\mathsf{Free}}
% \newcommand{\Preorder}{\mathsf{Preorder}}
% \newcommand{\CovTop}{\mathsf{Cov}}
% \newcommand{\Preshv}{\mathsf{PreShv}}
% \newcommand{\Precoshv}{\mathsf{PreCoshv}}
% \newcommand{\Ch}{\mathsf{Ch}}
% \newcommand{\grVect}{\mathsf{grVect}}

% \newcommand{\cat}{\mathsf{C}}
% \newcommand{\dat}{\mathsf{D}}
% \newcommand{\bat}{\mathsf{B}}
% \newcommand{\aat}{\mathsf{A}}
% \newcommand{\Lambdat}{\Lambda}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%    CATEGORIES  %%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Hom}{\mathrm{Hom}}
\newcommand{\obj}{\mathrm{obj}}
\newcommand{\mor}{\mathrm{mor}}
\newcommand{\Obj}{\mathrm{Obj}}
\newcommand{\Mor}{\mathrm{Mor}}
\newcommand{\Nat}{\mathrm{Nat}}
% \newcommand{\Hom}{\mathsf{Hom}}
% \newcommand{\obj}{\mathsf{obj}}
% \newcommand{\mor}{\mathsf{mor}}
% \newcommand{\Obj}{\mathsf{Obj}}
% \newcommand{\Mor}{\mathsf{Mor}}
% \newcommand{\Nat}{\mathsf{Nat}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\LocSys}{\mathbfsf{Loc}}
\newcommand{\Grp}{\mathbfsf{Grp}}
\newcommand{\Grpd}{\mathbfsf{Grpd}}
\newcommand{\SSet}{\mathbfsf{SSet}}
\newcommand{\Set}{\mathbfsf{Set}}
\newcommand{\Rel}{\mathbfsf{Rel}}
\newcommand{\Vect}{\mathbfsf{Vect}}
\newcommand{\vect}{\mathbfsf{vect}}
\newcommand{\Hilb}{\mathbfsf{Hilb}}
\newcommand{\Cat}{\mathbfsf{Cat}}
\newcommand{\Top}{\mathbfsf{Top}}
\newcommand{\hoTop}{\mathbfsf{hoTop}}
\newcommand{\Fun}{\mathbfsf{Fun}}
\newcommand{\Ab}{\mathbfsf{Ab}}
\newcommand{\Cov}{\mathbfsf{Cov}}
\newcommand{\Fincov}{\mathbfsf{FinCov}}
\newcommand{\Cell}{\mathbfsf{Cell}}
\newcommand{\Open}{\mathbfsf{Open}}
\newcommand{\Closed}{\mathbfsf{Closed}}
\newcommand{\Int}{\mathbfsf{Int}}
\newcommand{\Exit}{\mathbfsf{Exit}}
\newcommand{\Entr}{\mathbfsf{Entr}}
\newcommand{\Rep}{\mathbfsf{Rep}}
\newcommand{\Shv}{\mathbfsf{Shv}}
\newcommand{\Coshv}{\mathbfsf{CoShv}}
\newcommand{\Rout}{\mathbfsf{Rout}}
\newcommand{\Cone}{\mathbfsf{Cone}}
\newcommand{\CoCone}{\mathbfsf{CoCone}}
\newcommand{\Alex}{\mathbfsf{Alex}}
\newcommand{\Free}{\mathbfsf{Free}}
\newcommand{\Preorder}{\mathbfsf{Preorder}}
\newcommand{\CovTop}{\mathbfsf{Cov}}
\newcommand{\Preshv}{\mathbfsf{PreShv}}
\newcommand{\Precoshv}{\mathbfsf{PreCoshv}}
\newcommand{\Ch}{\mathbfsf{Ch}}
\newcommand{\grVect}{\mathbfsf{grVect}}

\newcommand{\cat}{\mathbfsf{C}}
\newcommand{\dat}{\mathbfsf{D}}
\newcommand{\bat}{\mathbfsf{B}}
\newcommand{\aat}{\mathbfsf{A}}
\newcommand{\Iat}{\mathbfsf{I}}
\newcommand{\Jat}{\mathbfsf{J}}
\newcommand{\Kat}{\mathbfsf{K}}
\newcommand{\Lambdat}{\boldsymbol{\Lambda}}
\newcommand{\pijuan}{\boldsymbol{\pi}_1}
\newcommand{\piinfty}{\boldsymbol{\pi}_{\infty}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   FUNCTORS  %%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\sheaf}{F}
\newcommand{\Sheaf}{F}
\newcommand{\Cech}{\check{C}}
\newcommand{\Leray}{L}
\newcommand{\SHom}{\mathcal{H}om}
\newcommand{\equivpc}{\mathcal{P}}
\newcommand{\equivqc}{\mathcal{Q}}
\newcommand{\cohomsheaf}{\mathcal{H}}
\newcommand{\covU}{\mathcal{U}}
\newcommand{\covS}{\mathcal{S}}
\newcommand{\covT}{\mathcal{T}}
\newcommand{\Loc}{\mathcal{L}}

\newcommand{\hF}{\widehat{F}}
\newcommand{\hG}{\widehat{G}}
\newcommand{\hP}{\widehat{P}}
\newcommand{\CHom}{\hat{\mathcal{H}}om}
\newcommand{\equivp}{\widehat{\mathcal{P}}}
\newcommand{\equivq}{\widehat{\mathcal{Q}}}
\newcommand{\cosec}{\widehat{\Gamma}}

\newcommand{\sk}{\mathbf{k}}
\newcommand{\csk}{\hat{\mathbf{k}}}
\newcommand{\ev}{\mathcal{E}}

\newcommand{\stalk}{\mathcal{S}}
\newcommand{\skycshv}{\hat{S}}
\newcommand{\skyshv}{S}
\newcommand{\Lan}{\mathrm{Lan}}
\newcommand{\Ran}{\mathrm{Ran}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Basic Constructions
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\id}{\mathrm{id}}
\newcommand{\colim}{\mathrm{colim}}
\newcommand{\pro}{\mathrm{pro}}
\newcommand{\coker}{\mathrm{coker}}
\newcommand{\cok}{\mathrm{cok}}
\newcommand{\im}{\mathrm{im}}
\newcommand{\Ext}{\mathrm{Ext}}
\newcommand{\Tor}{\mathrm{Tor}}
\newcommand{\inn}{\mathrm{in}}
\newcommand{\out}{\mathrm{out}}
\newcommand{\supp}{\mathrm{supp}}
\newcommand{\fr}{\mathrm{fr}}
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\Tot}{\mathrm{Tot}}
\newcommand{\st}{\mathrm{star}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% BOLD LETTERS
\newcommand{\bg}{{\bf g}}
\newcommand{\bh}{{\bf h}}
\newcommand{\bk}{{\bf k}}
\newcommand{\bq}{{\bf q}}
\newcommand{\bu}{{\bf u}}
\newcommand{\bv}{{\bf v}}
\newcommand{\bw}{{\bf w}}
\newcommand{\bx}{{\bf x}}
\newcommand{\by}{{\bf y}}
\newcommand{\bz}{{\bf z}}


\newcommand{\bA}{{\bf A}}
\newcommand{\bB}{{\bf B}}
\newcommand{\bC}{{\bf C}}
\newcommand{\bD}{{\bf D}}
\newcommand{\bF}{{\bf F}}
\newcommand{\bG}{{\bf G}}
\newcommand{\bM}{{\bf M}}
\newcommand{\bR}{{\bf R}}
\newcommand{\bI}{{\bf I}}


% BLACKBOARD BOLD LETTERS
%%%%%%%%%mathbb
\newcommand{\RR}{\mathbb{R}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\DD}{\mathbb{D}}
\newcommand{\BD}{\mathbb{D}}
\newcommand{\RP}{\mathbb{RP}}
\newcommand{\CP}{\mathbb{CP}}

\newcommand{\kk}{\mathbb{k}}

\newcommand{\HH}{\mathbb{H}}
\newcommand{\BB}{\mathbb{B}}

%\newcommand{\C}{{\mathbb{C}}}
\newcommand{\D}{{\mathbb{D}}}
\newcommand{\F}{{\mathbb{F}}}
\newcommand{\N}{{\mathbb{N}}}
\newcommand{\R}{{\mathbb{R}}}
\newcommand{\T}{{\mathbb{T}}}
\newcommand{\Z}{{\mathbb{Z}}}


% HOMOTOPY SYMBOL -- CHANGE THIS
\newcommand{\sh}{{\mathsf h}}

% FRAK LETTERS
%\newcommand{\cF}{{\mathfrak{f}}} % FOR MULTIVALUED MAPS

% CALIGRAPHIC LETTERS
\newcommand{\cA}{{\mathcal A}}
\newcommand{\cB}{{\mathcal B}}
\newcommand{\cC}{{\mathcal C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{{\mathcal E}}
\newcommand{\cF}{{\mathcal F}}
\newcommand{\cG}{{\mathcal G}}
\newcommand{\calG}{{\mathcal G}}
\newcommand{\cH}{{\mathcal H}}
\newcommand{\cI}{{\mathcal I}}
\newcommand{\cJ}{{\mathcal J}}
\newcommand{\cK}{{\mathcal K}}
\newcommand{\cL}{{\mathcal L}}
\newcommand{\cM}{{\mathcal M}}
\newcommand{\cN}{{\mathcal N}}
\newcommand{\cO}{{\mathcal O}}
\newcommand{\OO}{\mathcal{O}}
\newcommand{\cP}{{\mathcal P}}
\newcommand{\cQ}{{\mathcal Q}}
\newcommand{\cR}{{\mathcal R}}
\newcommand{\cS}{{\mathcal S}}
\newcommand{\cT}{{\mathcal T}}
\newcommand{\cU}{{\mathcal U}}
\newcommand{\cV}{{\mathcal V}}
\newcommand{\cW}{{\mathcal W}}
\newcommand{\cX}{{\mathcal X}}
\newcommand{\cY}{{\mathcal Y}}
\newcommand{\cZ}{{\mathcal Z}}

\newcommand{\cAKQ}{{\mathcal{AKQ}}}
\newcommand{\wed}{\mathop{w}\nolimits}
\newcommand{\ci}{{\mathsf{i}}}
\newcommand{\cj}{{\mathsf{j}}}

% San Serif LETTERS
\newcommand{\sA}{{\mathsf A}}
\newcommand{\sB}{{\mathsf B}}
\newcommand{\sC}{{\mathsf C}}
\newcommand{\sD}{{\mathsf D}}
\newcommand{\sE}{{\mathsf E}}
\newcommand{\sH}{{\mathsf H}}
\newcommand{\sI}{{\mathsf I}}
\newcommand{\sJ}{{\mathsf J}}
\newcommand{\sK}{{\mathsf K}}
\newcommand{\sL}{{\mathsf L}}
\newcommand{\sM}{{\mathsf M}}
\newcommand{\sN}{{\mathsf N}}
\newcommand{\sP}{{\mathsf P}}
\newcommand{\sQ}{{\mathsf Q}}
\newcommand{\sR}{{\mathsf R}}
\newcommand{\sT}{{\mathsf T}}
\newcommand{\sU}{{\mathsf U}}
\newcommand{\sV}{{\mathsf{V}}}
\newcommand{\sW}{{\mathsf W}}
\newcommand{\sZ}{{\mathsf Z}}

\newcommand{\src}{{\mathsf s}}
\newcommand{\tgt}{{\mathsf t}}


%\newcommand{\im}{{\mathsf i}}
\newcommand{\jm}{{\mathsf j}}
\newcommand{\km}{{\mathsf k}}
\newcommand{\lm}{{\mathsf l}}


\newcommand{\fF}{{\mathsf F}}
\newcommand{\fG}{{\mathsf G}}
\newcommand{\fH}{{\mathsf H}}
\newcommand{\fM}{{\mathsf M}}
\newcommand{\fS}{{\mathsf S}}
%%%%%%%%%% BOLD SAN SERIF
\newcommand{\bsA}{{\mathbfsf A}}
\newcommand{\bsB}{{\mathbfsf B}}
\newcommand{\bsC}{{\mathbfsf C}}
\newcommand{\bsD}{{\mathbfsf D}}
\newcommand{\bsE}{{\mathbfsf E}}
\newcommand{\bsF}{{\mathbfsf F}}
\newcommand{\bsG}{{\mathbfsf G}}
\newcommand{\bsH}{{\mathbfsf H}}
\newcommand{\bsI}{{\mathbfsf I}}
\newcommand{\bsJ}{{\mathbfsf J}}
\newcommand{\bsK}{{\mathbfsf K}}
\newcommand{\bsL}{{\mathbfsf L}}
%%alreadydefined%%\newcommand{\bsM}{{\mathbfsf M}}
\newcommand{\bsN}{{\mathbfsf N}}
\newcommand{\bsO}{{\mathbfsf O}}
\newcommand{\bsP}{{\mathbfsf P}}
\newcommand{\bsQ}{{\mathbfsf Q}}
\newcommand{\bsR}{{\mathbfsf R}}
%%alreadydefined%%\newcommand{\bsS}{{\mathbfsf S}}
\newcommand{\bsT}{{\mathbfsf T}}
\newcommand{\bsU}{{\mathbfsf U}}
\newcommand{\bsV}{{\mathbfsf V}}
\newcommand{\bsW}{{\mathbfsf W}}
\newcommand{\bsZ}{{\mathbfsf Z}}



\newcommand{\bjm}{{\mathbfsf j}}
\newcommand{\bkm}{{\mathbfsf k}}
\newcommand{\blm}{{\mathbfsf l}}



\newcommand{\bsM}{{\mathbfsf M}}
\newcommand{\bsS}{{\mathbfsf S}}

%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bs}{{\mathbf s}}
\newcommand{\be}{{\mathbf e}}

\newcommand{\ind}{{\text{ind}}}
\newcommand{\mul}{{\text{mul}}}


\newcommand{\Que}{{\sf{Que }}}

\newcommand{\setof}[1]{\left\{ {#1}\right\}}
\newcommand{\mvmap}{\raisebox{-0.2ex}{$\,\overrightarrow{\to}\,$}}
\newcommand{\setdef}[2]{\left\{{#1}\,\left|\,{#2}\right.\right\}}
\newcommand{\bdf}{\hbox{\rm bd$_f$}}
%\newcommand{\supp}[1]{\lfloor {#1}\rfloor}

\newcommand{\cb}{\mbox{\sf{cb}}}
\newcommand{\bd}{\mbox{\sf{bd}}}
\newcommand{\birth}{\text{\sf{b}}}

==> index.tex <==

CHAPTER 1 Categories

\index{category}
\index{category!small}\index{category!finite}
\index{category!discrete}
\index{relation}
\index{preordered set}
\index{poset}
\index{category!of open sets}
\index{category!of points and open sets}
\index{category!groupoid}\index{groupoid}
\index{category!fundamental groupoid}\index{fundamental groupoid}
\index{fundamental groupoid!Poincar\'e $\infty$-groupoid}
\index{category!data}\index{data types}
\index{category!subcategory}
\index{initial object}\index{terminal object}
\index{category!opposite}
\index{functor}
\index{natural transformation}
\index{naturally isomorphic}
\index{category!of functors}
\index{equivalence!adjoint}
\index{equivalence!fully faithful and essentially surjective}
\index{category!skeletal subcategory}\index{skeletal subcategory}
\index{diagram}
\index{representation}
\index{cones}
\index{cones!category of}\index{category!of cones}
\index{limit}
\index{limit!synonyms for}
\index{product}
\index{limit!is an intersection}
\index{pullback}
\index{equalizer}\index{kernel}
\index{invariants}
\index{cocones}
\index{cocones!category of}\index{category!of cocones} 
\index{colimit}
\index{colimit!synonyms for}
\index{coproduct}
\index{colimit!is a union}
\index{pushout}
\index{cokernel}\index{coequalizer}
\index{coinvariants}
\index{adjoint}
\index{adjoint!functor theorem, Freyd's}


CHAPTER 2 Theory of sheaves

\index{sheaf!three perspectives on}\index{cosheaf!three perspectives on}
\index{sheaf!on closed sets}
\index{cover}
\index{nerve}
\index{nerve theorem}
\index{presheaf}\index{pre-cosheaf}
\index{sheaf!definition of}\index{cosheaf!definition of}
\index{sheaf!axiom for two opens}\index{cosheaf!axiom for two opens}\index{cosheaf!of compactly supported functions}
\index{limit!over a cover}\index{colimit!over a cover}
\index{limit!as an equalizer}\index{colimit!as a coequalizer}
\index{sheaf!axiom as an equalizer}\index{cosheaf!axiom as a coequalizer}
\index{sheaf!axiom as an exact sequence}\index{cosheaf!axiom as an exact sequence}
\index{Cech@\v{C}ech homology}
\index{Cech@\v{C}ech homology!$\partial^2=0$}
\index{Cech@\v{C}ech homology!example of}
\index{cosheaf!Mayer-Vietoris}\index{Mayer-Vietoris}
\index{cosheaf!given by $H_0$}
\index{cover!refinement of}
\index{category!of covers}
\index{presheaf!behavior under refinement}\index{pre-cosheaf!behavior under refinement}
\index{sheaf!behavior under refinement}\index{cosheaf!behavior under refinement}
\index{sheaf!sheafification}
\index{sheaf!sheafification!universal property as a left adjoint}
\index{Grothendieck!Six Functor Formalism}
\index{sheaf!pushforward}
\index{presheaf!non-local example}
\index{presheaf!inconsistent example}
\index{stalk}\index{presheaf!stalk}\index{sheaf!stalk}
\index{product}\index{coproduct}\index{disjoint union}
\index{sheaf!pullback}\index{pullback!of sheaves}
\index{stalk}\index{sheaf!stalk}
\index{sheaf!Hom@$\SHom$}
\index{sheaf!tensor@$\otimes$}

\index{category!(co)filtered}
\index{category!of covers}
\index{limit!cofiltered}\index{colimit!filtered}
\index{costalk}\index{stalk}
\index{colimit!filtered!commutes with finite limits}
\index{exact!sequence of presheaves}\index{exact!sequence of sheaves}\index{sheaves!exact sequence of}\index{presheaf!exact sequence}
\index{limit!cofiltered!do not commute with finite colimits}
\index{category!opposite!of Vect@$\Vect$}
\index{sheaf!sheafification}
\index{cosheaf!cosheafification!approaches}
\index{cosheaf!cosheafification}
\index{cosheaf!cosheafification!universal property as a right adjoint}
\index{cosheaf!cosheafification!exists for Set@$\Set$}
\index{Vopenka's principle}

CHAPTER 3 PRELIMINARY EXAMPLES

\index{sheaf!of sections}
\index{fiber bundle}\index{covering space}
\index{M\"obius bundle}
\index{sheaf!constant sheaf}\index{sheaf!locally constant sheaf}
\index{local system}
\index{fiber byndle!gives local systems}\index{local system!from a fiber bundle}
\index{local system}\index{category! of local systems}
\index{local system! Klein bottle and torus examples}
\index{sheaf!locally constant sheaf}\index{cosheaf!locally constant cosheaf}
\index{local system!representation of $\pijuan(X)$}\index{fundamental groupoid!local systems}\index{representation!of fund@$\pijuan(X)$}
\index{sheaf!locally constant sheaf!representation of $\pijuan(X)$}\index{cosheaf!locally constant cosheaf!representation of $\pijuan(X)$}\index{fundamental groupoid $\pijuan(X)$!and locally constant (co)sheaves}index{representation!of fund@$\pijuan(X)$}
\index{van Kampen theorem}
\index{fundamental groupoid $\pijaun(X)$!determines locally constant (co)sheaves}
\index{cosheaf!of pre-images}
\index{cosheaf!of features}
\index{cosheaf!skyscraper}
\index{pointless topology}\index{locale}
\index{cosheaf!of connected components}
\index{cosheaf!of singular chains}
\index{Mayer-Vietoris and cosheaves}
\index{cosheaf!of compactly supported functions}
\index{Reeb graph}

CHAPTER 4 CELL SHEAVES

\index{regular cell complex}
\index{cell complex}
\index{cosheaf!cellular!height function on torus}
\index{category!of a cell complex $\Cell(X)$}
\index{stacks}
\index{cellular sheaves and cosheaves}\index{sheaf!cellular}\index{cosheaf!cellular}
\index{category!of cellular sheaves $\Shv(X)$, cosheaves $\Coshv(X)$}
\index{preordered set}\index{poset}
\index{Alexandrov topology}
\index{star}
\index{Alexandrov topology!unit interval example}
\index{Kan extension!motivation}
\index{Kan extension}
\index{sheaf!on a poset}\index{cosheaf!on a poset}
\index{sheaf!sections over a poset}\index{cosheaf!sections over a poset}
\index{cosheaf!on closed sets}\index{sheaf!on closed sets}

CHAPTER 5 FUNCTORS ASSOCIATED TO MAPS

\index{sheaf!pushforward}\index{cosheaf!pushforward}\index{direct image}
\index{poset!maps}
\index{pullback!of a sheaf over a poset}
\index{sheaf!constant sheaf!pullback from a point}
\index{subdivision}\index{cell complex!subdivision}
\index{subdivision!of a cellular sheaf}\index{sheaf!cellular!subdivision}
\index{global sections!pushforward to a point}\index{pushforward to a point}
\index{f@$f_{\dd}$ notation}
\index{pushforward with open supports $f_{\dd}$}\index{sheaf!pushforward $f_{\dd}$}
\index{cellular maps}
\index{pushforward with compact supports $f_!$}\index{sheaf!pushforward with compact supports $f_!$}
\index{cosheaf!pushforward with compact supports}
\index{cellular maps!projection to a point}
\index{cellular maps!inclusion of a point}
\index{cellular maps!bijection with a circle}
\index{sheaf!push-pull adjunctions}\index{cosheaf!push-pull adjunctions}

CHAPTER 6 HOMOLOGY AND COHOMOLOGY

\index{graded vector space}
\index{(co)chain complex}
\index{category!of chain complexes}
\index{cohomology}
\index{incidence relation}
\index{local orientation}
\index{cohomology!of a cell complex}
\index{cohomology!of a cellular sheaf!compactly-supported}\index{sheaf!cellular!compactly supported cohomology of}
\index{cohomology!of a cellular sheaf}\index{sheaf!cellular!cohomology of}
\index{homology!of a cellular cosheaf!Borel-Moore}\index{cosheaf!cellular!Borel-Moore homology of}
\index{homology!of a cellular cosheaf}\index{cosheaf!cellular!homology of}
\index{duality!linear}\index{linear duality}
\index{persistence module}\index{module!persistence}
\index{interval module}\index{module!interval}
\index{barcode}
\index{persistence module!decomposition theorem}\index{decomposition!barcode (interval)}
\index{barcode!length}
\index{barcode!fundamental theorem of linear algebra}
\index{barcode!filtration of Bott's torus}
\index{barcode!associated to chain complex}
\index{category!of representations}
\index{category!exact}
\index{exact!sequence of representations}
\index{representation!subrepresentation}
\index{representation!direct sum}
\index{category!additive}\index{category!abelian}
\index{representation!indecomposable}\index{indecomposable representation}
\index{splitting lemma}
\index{decomposition!Remak}
\index{Krull-Schmidt Theorem}
\index{indecomposable representation!constant (co)sheaves on connected}
\index{(co)chain complex!homotopy}
\index{quiver}
\index{category!path}
\index{quiver!representation}\index{representation!of a quiver}
\index{Gabriel's theorem}
\index{perversity}
\index{cellular perverse sheaves}\index{sheaf!cellular perverse}

CHAPTER 7 DERIVED PERSPECTIVE

\index{injective!objects}
\index{injective!properties}
\index{sheaf!elementary injective cellular sheaf $[\sigma]^W$}\index{injective!cellular sheaf}
\index{injective!sheaf on a poset}\index{sheaf! elementary injective on a poset}\index{injective!cosheaf on a poset}\index{cosheaf!elementary injective on a poset}
\index{injective!cellular sheaves are sums}
\index{projective!objects}
\index{projective!properties}
\index{projective!sheaf on a poset}\index{sheaf! elementary projective on a poset}\index{projective!cosheaf on a poset}\index{cosheaf!elementary projective on a poset}
\index{injective!mapping identities for (co)sheaves}
\index{projective!mapping identities for (co)sheaves}
\index{injective!resolutions}\index{projective!resolutions}
\index{category!C@$C^b(\aat)$ of chain complexes}\index{category!K@$K^b(\aat)$ homotopy category of chain complexes}\index{H@$K^b(\aat)$ homotopy category of chain complexes}
\index{Derived@$D^b(\aat)$ derived category}\index{category!Derived@$D^b(\aat)$ derived category}
\index{quasi-isomorphism}
\index{Left@$Lf_*$ left derived pushforward}
\index{cosheaf!cellular homology!Left@$Lf_*$ left derived pushforward}
\index{Borel-Moore cosheaf homology}\index{cosheaf!cellular!Borel-Moore homology}
\index{Borel-Moore cosheaf homology!invariance under subdivision}\index{cosheaf!cellular!Borel-Moore homology under subdivision}
\index{sheaf!homology, cellular}\index{cosheaf!cohomology, cellular}
\index{duality!over a manifold}

CHAPTER 8 TDA

\index{point cloud}\index{persistent homology}
\index{persistent homology!sublevel set}
\index{category!of intervals}
\index{persistent homology!level set/zigzag}
\index{absolute homology cosheaf}\index{cosheaf!absolute homology}
\index{homology!of a cellular cosheaf!via barcodes}\index{cosheaf!cellular!homology via barcodes}
\index{barcode!trick}
\index{discrete Morse theory for sheaves}
\index{nerve theorem}
\index{sheaf!C@\v{C}ech}\index{Cech@\v{C}ech sheaves}
\index{Mayer-Vietoris!via cellular sheaf cohomology}
\index{sheaf!Leray}\index{Leray sheaves}
\index{Mayer-Vietoris!blowup complex}\index{nerve!generalization}
\index{nerve theorem!generalization}
\index{persistent homology!level set determines sublevel set}
\index{persistent homology!multi-dimensional!sublevel set}
\index{persistent homology!multi-dimensional!via derived pushforward}
\index{barcode!generalized}\index{decomposition!generalized barcode}

CHAPTER 9 NC CODING

\index{quiver}\index{graph}
\index{capacity}
\index{network coding sheaf}\index{sheaf!network coding}
\index{routing sheaf}\index{sheaf!routing}
\index{duality!for routing sheaves}\index{routing sheaf!duality}
\index{duality!network coding sheaf}\index{network coding sheaf!duality}
\index{decoding edge}
\index{sheaf!homology, cellular!examples}

CHAPTER 10 SENSORS

\index{sensors}
\index{intruder problem}
\index{intruder problem!approaches to}
\index{sensors!multi-modal}
\index{sensing sheaf}\index{sheaf!sensing}
\index{evasion cosheaf}\index{cosheaf!evasion}
\index{decomposition!sensing and evasion regions}

CHAPTER 11 ENTRANCE PATH CATEGORY

\index{sheaf!constructible}\index{sheaf!restricted sheaf}\index{cosheaf!constructible}
\index{decomposition!into strata}\index{strata}
\index{blowup map}
\index{stratified space!Whitney}
\index{stratified space!general properties of}
\index{stratified map!Whitney}
\index{stratified submersion}
\index{Thom's first isotopy lemma}
\index{tame topology}
\index{o-minimal structure}
\index{semialgebraic subset}
\index{analytic-geometric category}\index{o-minimal structure!analytic-geometric category}
\index{control data}
\index{stratified space!Thom-Mather}
\index{family of lines}
\index{strata!closed union, has regular neighborhood}
\index{stratified vector field}
\index{stratified map!Thom mapping}
\index{point cloud!determines a stratified map}
\index{entrance path category}
\index{entrance path category!definable}\index{definable entrance path category}
\index{category!skeletal subcategory}\index{skeletal subcategory
\index{Entr@$\Entr(X)$ entrance path category!representations are cosheaves}\index{representation!of Entr@$\Entr(X)$}
\index{cosheaf!constructible!is representation of entr@$\Entr(X)$}
\index{cosheaf!constructible!from a definable map}\index{stratified map!determines constructible cosheaves}\index{representation!of entr@$\Entr(X)$! from a stratified map

CHAPTER 12 DUALITY

\index{duality!Poincar\'e-Verdier equivalence functor}
\index{duality!over a manifold}
\index{duality!derived equivalence}\index{derived equivalence!of cellular sheaves and cosheaves}\index{sheaf!cellular!derived equivalence with cosheaves}\index{cosheaf!cellular!derived equivalence with sheaves}
\index{duality!linear}\index{linear duality}
\index{Verdier duality}\index{duality!Verdier}

CHAPTER 13 VALUATIONS

\index{module!left and right}
\index{coend}\index{tensoring sheaves with cosheaves}
\index{Pitt's theorem}
\index{cohomology!of a cellular sheaf!compactly-supported}\index{sheaf!cellular!compactly supported cohomology of
\index{sheaf!homology, cellular}
\index{coend!higher Euler calculus

CHAPTER 14 GRADED 

\index{barcode!associated to chain complex}
\index{derived equivalence!with graded vector spaces}
\index{Derived@$D^b(\aat)$ derived category!calculus of fractions}\index{category!Derived@$D^b(\aat)$ derived category!calculus of fractions}
\index{derived equivalence!with graded sheaves}\index{sheaf!cellular!derived equivalence with graded sheaves}

CHAPTER 15 METRIC

\index{epsilon@$\epsilon$ thickening}
\index{interleaving!of presheaves}
\index{stability}
\index{interleaving!of presheaves!obstructed by global sections
\index{interleaving!sheaves}
\index{stability!for derived interleavings}
\index{category!of definable sheaves}\index{sheaf!definable}
\index{interleaving!of sheaves!over the real line}
\index{category!of sheaves!coordinates}
\index{bottleneck distance}
